A crystallographic approach to symmetry-breaking in fluid layers

Symmetry-breaking bifurcations, where a flow state with a certain symmetry undergoes a transition to state with a different symmetry, are ubiquitous in fluid mechanics. Much can be understood about the nature of these transitions from symmetry alone, using the theory of groups and their representations. Here we show how the extensive databases on groups in crystallography can be exploited to yield insights into fluid-dynamical problems. In particular, we demonstrate the application of the crystallographic layer groups to problems in fluid layers, using thermal convection as an example. Crystallographic notation provides a concise and unambiguous description of the symmetries involved, and we advocate its broader use by the fluid dynamics community.

==> cryst_char.tex <==
\begin{table}[!ht]
\centering
\caption{Character table of $p1$ (No. 1)}
\begin{tabular}{r|r|l}
\toprule
 & $1$ & axial subgroups \\
\midrule
size & 1 &  \\ \midrule
$A_{}$ & $1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{1}$ (No. 2)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $\overline{1}$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p112$ (No. 3)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $2_z$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $p112$ (3) \\
$B_{}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p11m$ (No. 4)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{}^\prime$ & $1$ & $1$ & $p11m$ (4) \\
$A_{}^{\prime\prime}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p11a$ (No. 5)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{}^\prime$ & $1$ & $1$ & $p11a$ (5) \\
$A_{}^{\prime\prime}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p112/m$ (No. 6)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{1}$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $p112/m$ (6) \\
$B_{g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{u}$ & $1$ & $-1$ & $-1$ & $1$ & $p11m$ (4) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p112/a$ (No. 7)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{1}$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $p112/a$ (7) \\
$B_{g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{u}$ & $1$ & $-1$ & $-1$ & $1$ & $p11a$ (5) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p211$ (No. 8)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $p211$ (8) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2_111$ (No. 9)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $p2_111$ (9) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $c211$ (No. 10)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $c211$ (10) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm11$ (No. 11)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $pm11$ (11) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pb11$ (No. 12)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $pb11$ (12) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cm11$ (No. 13)}
\begin{tabular}{r|rr|l}
\toprule
 & $1$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $cm11$ (13) \\
$A_{2}$ & $1$ & $-1$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2/m11$ (No. 14)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $\overline{1}$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $p2/m11$ (14) \\
$A_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2_1/m11$ (No. 15)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $\overline{1}$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $p2_1/m11$ (15) \\
$A_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2/b11$ (No. 16)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $\overline{1}$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $p2/b11$ (16) \\
$A_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2_1/b11$ (No. 17)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $\overline{1}$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $p2_1/b11$ (17) \\
$A_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $c2/m11$ (No. 18)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $\overline{1}$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $c2/m11$ (18) \\
$A_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $p\overline{1}$ (2) \\
$A_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $c211$ (10) \\
$A_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p222$ (No. 19)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $p222$ (19) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{2}$ & $1$ & $-1$ & $1$ & $-1$ & $p211$ (8) \\
$B_{3}$ & $1$ & $-1$ & $-1$ & $1$ & $p211$ (8) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2_122$ (No. 20)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_x$ & $2_y$ & $2_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $p2_122$ (20) \\
$B_{1}$ & $1$ & $-1$ & $-1$ & $1$ & $p112$ (3) \\
$B_{2}$ & $1$ & $-1$ & $1$ & $-1$ & $p211$ (8) \\
$B_{3}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p2_12_12$ (No. 21)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $p2_12_12$ (21) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{2}$ & $1$ & $-1$ & $1$ & $-1$ & $p2_111$ (9) \\
$B_{3}$ & $1$ & $-1$ & $-1$ & $1$ & $p2_111$ (9) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $c222$ (No. 22)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $c222$ (22) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{2}$ & $1$ & $-1$ & $1$ & $-1$ & $c211$ (10) \\
$B_{3}$ & $1$ & $-1$ & $-1$ & $1$ & $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmm2$ (No. 23)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $pmm2$ (23) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{1}$ & $1$ & $-1$ & $1$ & $-1$ & $pm11$ (11) \\
$B_{2}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pma2$ (No. 24)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $pma2$ (24) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{1}$ & $1$ & $-1$ & $1$ & $-1$ & $pb11$ (12) \\
$B_{2}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pba2$ (No. 25)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $pba2$ (25) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{1}$ & $1$ & $-1$ & $1$ & $-1$ & $pb11$ (12) \\
$B_{2}$ & $1$ & $-1$ & $-1$ & $1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cmm2$ (No. 26)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $cmm2$ (26) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$B_{1}$ & $1$ & $-1$ & $1$ & $-1$ & $cm11$ (13) \\
$B_{2}$ & $1$ & $-1$ & $-1$ & $1$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm2m$ (No. 27)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pm2m$ (27) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2}^\prime$ & $1$ & $-1$ & $-1$ & $1$ & $p11m$ (4) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $1$ & $-1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm2_1b$ (No. 28)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pm2_1b$ (28) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2}^\prime$ & $1$ & $-1$ & $1$ & $-1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm2_1m$ (No. 29)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pm2_1m$ (29) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2}^\prime$ & $1$ & $-1$ & $-1$ & $1$ & $p11m$ (4) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $1$ & $-1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pb2b$ (No. 30)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pb2b$ (30) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2}^\prime$ & $1$ & $-1$ & $1$ & $-1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $-1$ & $1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm2a$ (No. 31)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pm2a$ (31) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2}^\prime$ & $1$ & $-1$ & $1$ & $-1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pm2_1n$ (No. 32)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pm2_1n$ (32) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2}^\prime$ & $1$ & $-1$ & $1$ & $-1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $-1$ & $1$ & $pm11$ (11) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pb2_1a$ (No. 33)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pb2_1a$ (33) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p2_111$ (9) \\
$A_{2}^\prime$ & $1$ & $-1$ & $1$ & $-1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $-1$ & $1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pb2n$ (No. 34)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $pb2n$ (34) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $p211$ (8) \\
$A_{2}^\prime$ & $1$ & $-1$ & $-1$ & $1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $1$ & $-1$ & $pb11$ (12) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cm2m$ (No. 35)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $cm2m$ (35) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $c211$ (10) \\
$A_{2}^\prime$ & $1$ & $-1$ & $-1$ & $1$ & $p11m$ (4) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $1$ & $-1$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cm2e$ (No. 36)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $cm2e$ (36) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $c211$ (10) \\
$A_{2}^\prime$ & $1$ & $-1$ & $-1$ & $1$ & $p11a$ (5) \\
$A_{2}^{\prime\prime}$ & $1$ & $-1$ & $1$ & $-1$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmmm$ (No. 37)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pmmm$ (37) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/m$ (6) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2/m11$ (14) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2/m11$ (14) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p222$ (19) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pmm2$ (23) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pm2m$ (27) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2m$ (27) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmaa$ (No. 38)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_x$ & $2_z$ & $2_y$ & $\overline{1}$ & $m_x$ & $m_z$ & $m_y$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pmaa$ (38) \\
$B_{1g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2/b11$ (16) \\
$B_{3g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p2/m11$ (14) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p222$ (19) \\
$B_{1u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pma2$ (24) \\
$B_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2a$ (31) \\
$B_{3u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pb2b$ (30) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pban$ (No. 39)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pban$ (39) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2/b11$ (16) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2/b11$ (16) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p222$ (19) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pba2$ (25) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pb2n$ (34) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pb2n$ (34) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmam$ (No. 40)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_y$ & $2_z$ & $2_x$ & $\overline{1}$ & $m_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pmam$ (40) \\
$B_{1g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p112/m$ (6) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p2/b11$ (16) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2_1/m11$ (15) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_122$ (20) \\
$B_{1u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pma2$ (24) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pm2m$ (27) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2_1m$ (29) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmma$ (No. 41)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pmma$ (41) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2/m11$ (14) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2_1/m11$ (15) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_122$ (20) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pmm2$ (23) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pm2a$ (31) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2_1b$ (28) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pman$ (No. 42)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_y$ & $2_z$ & $2_x$ & $\overline{1}$ & $m_y$ & $m_z$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pman$ (42) \\
$B_{1g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p2_1/b11$ (17) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2/m11$ (14) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_122$ (20) \\
$B_{1u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pma2$ (24) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pm2_1n$ (32) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pb2n$ (34) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pbaa$ (No. 43)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_x$ & $2_z$ & $2_y$ & $\overline{1}$ & $m_x$ & $m_z$ & $m_y$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pbaa$ (43) \\
$B_{1g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2_1/b11$ (17) \\
$B_{3g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p2/b11$ (16) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_122$ (20) \\
$B_{1u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pba2$ (25) \\
$B_{2u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pb2_1a$ (33) \\
$B_{3u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pb2b$ (30) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pbam$ (No. 44)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pbam$ (44) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/m$ (6) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2_1/b11$ (17) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2_1/b11$ (17) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_12_12$ (21) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pba2$ (25) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pm2_1m$ (29) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2_1m$ (29) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pbma$ (No. 45)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_y$ & $2_x$ & $2_z$ & $\overline{1}$ & $m_y$ & $m_x$ & $m_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pbma$ (45) \\
$B_{1g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p2_1/m11$ (15) \\
$B_{3g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2_1/b11$ (17) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_12_12$ (21) \\
$B_{1u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pma2$ (24) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pb2_1a$ (33) \\
$B_{3u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pm2_1b$ (28) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $pmmn$ (No. 46)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $pmmn$ (46) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $p2_1/m11$ (15) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $p2_1/m11$ (15) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p2_12_12$ (21) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $pmm2$ (23) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $pm2_1n$ (32) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $pm2_1n$ (32) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cmmm$ (No. 47)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $cmmm$ (47) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/m$ (6) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $c2/m11$ (18) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c2/m11$ (18) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $c222$ (22) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $cmm2$ (26) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $cm2m$ (35) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $cm2m$ (35) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $cmme$ (No. 48)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $2_y$ & $2_x$ & $\overline{1}$ & $m_z$ & $m_y$ & $m_x$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $cmme$ (48) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/a$ (7) \\
$B_{2g}$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $-1$ & $c2/m11$ (18) \\
$B_{3g}$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c2/m11$ (18) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $c222$ (22) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $cmm2$ (26) \\
$B_{2u}$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $cm2e$ (36) \\
$B_{3u}$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $cm2e$ (36) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4$ (No. 49)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $4_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $p4$ (49) \\
$B_{}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$^1E_{}$ & $1$ & $-1$ & $-i$ & $i$ & $p1$ (1) \\
$^2E_{}$ & $1$ & $-1$ & $i$ & $-i$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{4}$ (No. 50)}
\begin{tabular}{r|rrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{4}_z$ & $\overline{4}_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $p\overline{4}$ (50) \\
$B_{}$ & $1$ & $1$ & $-1$ & $-1$ & $p112$ (3) \\
$^1E_{}$ & $1$ & $-1$ & $-i$ & $i$ & $p1$ (1) \\
$^2E_{}$ & $1$ & $-1$ & $i$ & $-i$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/m$ (No. 51)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $4_z^{-1}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $\overline{4}_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/m$ (51) \\
$B_{g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/m$ (6) \\
$^1E_{g}$ & $1$ & $-1$ & $-i$ & $i$ & $1$ & $-1$ & $-i$ & $i$ & $p\overline{1}$ (2) \\
$^2E_{g}$ & $1$ & $-1$ & $i$ & $-i$ & $1$ & $-1$ & $i$ & $-i$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p\overline{4}$ (50) \\
$^1E_{u}$ & $1$ & $-1$ & $-i$ & $i$ & $-1$ & $1$ & $i$ & $-i$ & $p11m$ (4) \\
$^2E_{u}$ & $1$ & $-1$ & $i$ & $-i$ & $-1$ & $1$ & $-i$ & $i$ & $p11m$ (4) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/n$ (No. 52)}
\begin{tabular}{r|rrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $4_z^{-1}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $\overline{4}_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/n$ (52) \\
$B_{g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $p112/a$ (7) \\
$^1E_{g}$ & $1$ & $-1$ & $-i$ & $i$ & $1$ & $-1$ & $-i$ & $i$ & $p\overline{1}$ (2) \\
$^2E_{g}$ & $1$ & $-1$ & $i$ & $-i$ & $1$ & $-1$ & $i$ & $-i$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p\overline{4}$ (50) \\
$^1E_{u}$ & $1$ & $-1$ & $-i$ & $i$ & $-1$ & $1$ & $i$ & $-i$ & $p11a$ (5) \\
$^2E_{u}$ & $1$ & $-1$ & $i$ & $-i$ & $-1$ & $1$ & $-i$ & $i$ & $p11a$ (5) \\
\bottomrule
\end{tabular}
\end{table}
\clearpage
\begin{table}[!ht]
\centering
\caption{Character table of $p422$ (No. 53)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p422$ (53) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $p222$ (19) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c222$ (22) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p211$ (8), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p42_12$ (No. 54)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p42_12$ (54) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $p2_12_12$ (21) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c222$ (22) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2_111$ (9), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4mm$ (No. 55)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4mm$ (55) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pmm2$ (23) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmm2$ (26) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $pm11$ (11), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4bm$ (No. 56)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4bm$ (56) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4$ (49) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pba2$ (25) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmm2$ (26) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $pb11$ (12), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{4}2m$ (No. 57)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{4}_z$ & $2_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{4}2m$ (57) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{4}$ (50) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $p222$ (19) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmm2$ (26) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p211$ (8), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{4}2_1m$ (No. 58)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{4}_z$ & $2_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{4}2_1m$ (58) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{4}$ (50) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $p2_12_12$ (21) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmm2$ (26) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2_111$ (9), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{4}m2$ (No. 59)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{4}_z$ & $m_y$ & $2_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{4}m2$ (59) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{4}$ (50) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c222$ (22) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pmm2$ (23) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $pm11$ (11), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{4}b2$ (No. 60)}
\begin{tabular}{r|rrrrr|l}
\toprule
 & $1$ & $2_z$ & $\overline{4}_z$ & $m_y$ & $2_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{4}b2$ (60) \\
$A_{2}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{4}$ (50) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $c222$ (22) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pba2$ (25) \\
$E_{}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $pb11$ (12), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/mmm$ (No. 61)}
\begin{tabular}{r|rrrrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/mmm$ (61) \\
$A_{2g}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4/m$ (51) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pmmm$ (37) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmmm$ (47) \\
$E_{g}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2/m11$ (14), $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p422$ (53) \\
$A_{2u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p4mm$ (55) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $p\overline{4}2m$ (57) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{4}m2$ (59) \\
$E_{u}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $-2$ & $2$ & $0$ & $0$ & $0$ & $pm2m$ (27), $cm2m$ (35) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/nbm$ (No. 62)}
\begin{tabular}{r|rrrrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/nbm$ (62) \\
$A_{2g}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4/n$ (52) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pban$ (39) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmme$ (48) \\
$E_{g}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2/b11$ (16), $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p422$ (53) \\
$A_{2u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p4bm$ (56) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $p\overline{4}2m$ (57) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{4}b2$ (60) \\
$E_{u}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $-2$ & $2$ & $0$ & $0$ & $0$ & $pb2n$ (34), $cm2e$ (36) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/mbm$ (No. 63)}
\begin{tabular}{r|rrrrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/mbm$ (63) \\
$A_{2g}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4/m$ (51) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pbam$ (44) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmmm$ (47) \\
$E_{g}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2_1/b11$ (17), $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p42_12$ (54) \\
$A_{2u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p4bm$ (56) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $p\overline{4}2_1m$ (58) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{4}b2$ (60) \\
$E_{u}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $-2$ & $2$ & $0$ & $0$ & $0$ & $pm2_1m$ (29), $cm2m$ (35) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p4/nmm$ (No. 64)}
\begin{tabular}{r|rrrrrrrrrr|l}
\toprule
 & $1$ & $2_z$ & $4_z$ & $2_y$ & $2_{xy}$ & $\overline{1}$ & $m_z$ & $\overline{4}_z$ & $m_y$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 1 & 2 & 2 & 2 & 1 & 1 & 2 & 2 & 2 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p4/nmm$ (64) \\
$A_{2g}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p4/n$ (52) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $pmmn$ (46) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $cmme$ (48) \\
$E_{g}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $p2_1/m11$ (15), $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p42_12$ (54) \\
$A_{2u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p4mm$ (55) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $p\overline{4}2_1m$ (58) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{4}m2$ (59) \\
$E_{u}$ & $2$ & $-2$ & $0$ & $0$ & $0$ & $-2$ & $2$ & $0$ & $0$ & $0$ & $pm2_1n$ (32), $cm2e$ (36) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p3$ (No. 65)}
\begin{tabular}{r|rrr|l}
\toprule
 & $1$ & $3_z$ & $3_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $p3$ (65) \\
$^1E_{}$ & $1$ & $\omega^2$ & $\omega$ & $p1$ (1) \\
$^2E_{}$ & $1$ & $\omega$ & $\omega^2$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{3}$ (No. 66)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $3_z^{-1}$ & $\overline{1}$ & $\overline{3}_z$ & $\overline{3}_z^{-1}$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{3}$ (66) \\
$^1E_{g}$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $p\overline{1}$ (2) \\
$^2E_{g}$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $p\overline{1}$ (2) \\
$A_{u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p3$ (65) \\
$^1E_{u}$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $p1$ (1) \\
$^2E_{u}$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p312$ (No. 67)}
\begin{tabular}{r|rrr|l}
\toprule
 & $1$ & $3_z$ & $2_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $p312$ (67) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $p3$ (65) \\
$E_{}$ & $2$ & $-1$ & $0$ & $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p321$ (No. 68)}
\begin{tabular}{r|rrr|l}
\toprule
 & $1$ & $3_z$ & $2_{xy}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $p321$ (68) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $p3$ (65) \\
$E_{}$ & $2$ & $-1$ & $0$ & $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p3m1$ (No. 69)}
\begin{tabular}{r|rrr|l}
\toprule
 & $1$ & $3_z$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $p3m1$ (69) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $p3$ (65) \\
$E_{}$ & $2$ & $-1$ & $0$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p31m$ (No. 70)}
\begin{tabular}{r|rrr|l}
\toprule
 & $1$ & $3_z$ & $m_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $p31m$ (70) \\
$A_{2}$ & $1$ & $1$ & $-1$ & $p3$ (65) \\
$E_{}$ & $2$ & $-1$ & $0$ & $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{3}1m$ (No. 71)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $2_{3}$ & $\overline{1}$ & $\overline{3}_z$ & $m_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 & 1 & 2 & 3 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{3}1m$ (71) \\
$A_{2g}$ & $1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{3}$ (66) \\
$E_{g}$ & $2$ & $-1$ & $0$ & $2$ & $-1$ & $0$ & $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p312$ (67) \\
$A_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p31m$ (70) \\
$E_{u}$ & $2$ & $-1$ & $0$ & $-2$ & $1$ & $0$ & $c211$ (10), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{3}m1$ (No. 72)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $2_{xy}$ & $\overline{1}$ & $\overline{3}_z$ & $m_{xy}$ & axial subgroups \\
\midrule
size & 1 & 2 & 3 & 1 & 2 & 3 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{3}m1$ (72) \\
$A_{2g}$ & $1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $p\overline{3}$ (66) \\
$E_{g}$ & $2$ & $-1$ & $0$ & $2$ & $-1$ & $0$ & $c2/m11$ (18) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p321$ (68) \\
$A_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p3m1$ (69) \\
$E_{u}$ & $2$ & $-1$ & $0$ & $-2$ & $1$ & $0$ & $c211$ (10), $cm11$ (13) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p6$ (No. 73)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $3_z^{-1}$ & $2_z$ & $6_z^{-1}$ & $6_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p6$ (73) \\
$B_{}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p3$ (65) \\
$^1E_{1}$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $p1$ (1) \\
$^2E_{1}$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $p1$ (1) \\
$^1E_{2}$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $p112$ (3) \\
$^2E_{2}$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $p112$ (3) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{6}$ (No. 74)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $3_z^{-1}$ & $m_z$ & $\overline{6}_z^{-1}$ & $\overline{6}_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{}^\prime$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{6}$ (74) \\
$A_{}^{\prime\prime}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p3$ (65) \\
$^1E_{}^\prime$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $p11m$ (4) \\
$^2E_{}^\prime$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $p11m$ (4) \\
$^1E_{}^{\prime\prime}$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $p1$ (1) \\
$^2E_{}^{\prime\prime}$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $p1$ (1) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p6/m$ (No. 75)}
\begin{tabular}{r|rrrrrrrrrrrr|l}
\toprule
 & $1$ & $3_z$ & $3_z^{-1}$ & $2_z$ & $6_z^{-1}$ & $6_z$ & $\overline{1}$ & $\overline{3}_z$ & $\overline{3}_z^{-1}$ & $m_z$ & $\overline{6}_z^{-1}$ & $\overline{6}_z$ & axial subgroups \\
\midrule
size & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &  \\ \midrule
$A_{g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p6/m$ (75) \\
$B_{g}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $p\overline{3}$ (66) \\
$^1E_{1g}$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $p\overline{1}$ (2) \\
$^2E_{1g}$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $p\overline{1}$ (2) \\
$^1E_{2g}$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $p112/m$ (6) \\
$^2E_{2g}$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $p112/m$ (6) \\
$A_{u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p6$ (73) \\
$B_{u}$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $p\overline{6}$ (74) \\
$^1E_{1u}$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $1$ & $\omega^2$ & $\omega$ & $p11m$ (4) \\
$^2E_{1u}$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $p11m$ (4) \\
$^1E_{2u}$ & $1$ & $\omega^2$ & $\omega$ & $1$ & $\omega^2$ & $\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $-1$ & $-\omega^2$ & $-\omega$ & $p112$ (3) \\
$^2E_{2u}$ & $1$ & $\omega$ & $\omega^2$ & $1$ & $\omega$ & $\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $-1$ & $-\omega$ & $-\omega^2$ & $p112$ (3) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p622$ (No. 76)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $2_z$ & $6_z$ & $2_{xy}$ & $2_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 1 & 2 & 3 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p622$ (76) \\
$A_{2}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p6$ (73) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $p321$ (68) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p312$ (67) \\
$E_{1}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $c211$ (10), $c211$ (10) \\
$E_{2}$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $c222$ (22) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p6mm$ (No. 77)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $2_z$ & $6_z$ & $m_{xy}$ & $m_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 1 & 2 & 3 & 3 &  \\ \midrule
$A_{1}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p6mm$ (77) \\
$A_{2}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p6$ (73) \\
$B_{1}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $p3m1$ (69) \\
$B_{2}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p31m$ (70) \\
$E_{1}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $cm11$ (13), $cm11$ (13) \\
$E_{2}$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $cmm2$ (26) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{6}m2$ (No. 78)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $m_z$ & $\overline{6}_z$ & $m_{xy}$ & $2_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 1 & 2 & 3 & 3 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{6}m2$ (78) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p312$ (67) \\
$A_{2}^\prime$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{6}$ (74) \\
$A_{2}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $p3m1$ (69) \\
$E_{}^\prime$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $cm2m$ (35) \\
$E_{}^{\prime\prime}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $cm11$ (13), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p\overline{6}2m$ (No. 79)}
\begin{tabular}{r|rrrrrr|l}
\toprule
 & $1$ & $3_z$ & $m_z$ & $\overline{6}_z$ & $2_{xy}$ & $m_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 1 & 2 & 3 & 3 &  \\ \midrule
$A_{1}^\prime$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p\overline{6}2m$ (79) \\
$A_{1}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $p321$ (68) \\
$A_{2}^\prime$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p\overline{6}$ (74) \\
$A_{2}^{\prime\prime}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p31m$ (70) \\
$E_{}^\prime$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $cm2m$ (35) \\
$E_{}^{\prime\prime}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $cm11$ (13), $c211$ (10) \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!ht]
\centering
\caption{Character table of $p6/mmm$ (No. 80)}
\begin{tabular}{r|rrrrrrrrrrrr|l}
\toprule
 & $1$ & $3_z$ & $2_z$ & $6_z$ & $2_{xy}$ & $2_{3}$ & $\overline{1}$ & $\overline{3}_z$ & $m_z$ & $\overline{6}_z$ & $m_{xy}$ & $m_{3}$ & axial subgroups \\
\midrule
size & 1 & 2 & 1 & 2 & 3 & 3 & 1 & 2 & 1 & 2 & 3 & 3 &  \\ \midrule
$A_{1g}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $p6/mmm$ (80) \\
$A_{2g}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $p6/m$ (75) \\
$B_{1g}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $p\overline{3}m1$ (72) \\
$B_{2g}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $p\overline{3}1m$ (71) \\
$E_{1g}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $c2/m11$ (18), $c2/m11$ (18) \\
$E_{2g}$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $cmmm$ (47) \\
$A_{1u}$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $p622$ (76) \\
$A_{2u}$ & $1$ & $1$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $p6mm$ (77) \\
$B_{1u}$ & $1$ & $1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $1$ & $-1$ & $1$ & $p\overline{6}2m$ (79) \\
$B_{2u}$ & $1$ & $1$ & $-1$ & $-1$ & $-1$ & $1$ & $-1$ & $-1$ & $1$ & $1$ & $1$ & $-1$ & $p\overline{6}m2$ (78) \\
$E_{1u}$ & $2$ & $-1$ & $-2$ & $1$ & $0$ & $0$ & $-2$ & $1$ & $2$ & $-1$ & $0$ & $0$ & $cm2m$ (35), $cm2m$ (35) \\
$E_{2u}$ & $2$ & $-1$ & $2$ & $-1$ & $0$ & $0$ & $-2$ & $1$ & $-2$ & $1$ & $0$ & $0$ & $cmm2$ (26), $c222$ (22) \\
\bottomrule
\end{tabular}
\end{table}

